Improving Streaming Speech Recognition With Time-Shifted Contextual Attention And Dynamic Right Context Masking

Chunk-based inference stands out as a popular approach in developing real-time streaming speech recognition, valued for its simplicity and efficiency. However, because it restricts the model's focus to only the history and current chunk context, it may result in performance degradation in scenarios that demand consideration of future context. Addressing this, we propose a novel approach featuring Time-Shifted Contextual Attention (TSCA) and Dynamic Right Context (DRC) masking. Our method shows a relative word error rate reduction of 10 to 13.9% on the Librispeech dataset with the inclusion of in-context future information provided by TSCA. Moreover, we present a streaming automatic speech recognition pipeline that facilitates the integration of TSCA with minimal user-perceived latency, while also enabling batch processing capability, making it practical for various applications.

==> lor.tex <==
Chau Thanh Duc,
Head, Zalo AI Laboratory
ctduc@fit.hcmus.edu.vn
13/4/2024

Sponsorship Committee
Interspeech 2024

Dear Members of the Sponsorship Committee,

I am writing to recommend Le Duy Khanh, a talented young researcher from our Zalo AI Laboratory, for sponsorship to attend Interspeech 2024 in Greece. His paper, titled "Improving Streaming Speech Recognition with Time-Shifted Contextual Attention and Dynamic Right Context Masking" (Paper ID: 1971), has been accepted for presentation at the conference, receiving positive reviews (Accept - Accept - Weak accept).

Khanh is an early-career researcher who has shown exceptional dedication and promise in the field of speech recognition. His accepted paper is a testament to his innovative approach and hard work. This achievement is particularly significant given that it is his first research paper. Attending Interspeech would provide him invaluable exposure to the global research community, allowing him to gain insights, network with experts, and receive constructive feedback on his work.

However, as a laboratory based in Vietnam, a less-represented and low-income country, we face considerable financial constraints. The overall participation costs for Interspeech in Greece are significant, nearly equivalent to Khanh's annual income. Our current funding is insufficient to cover the expenses of international travel to the conference. Unfortunately, our efforts to secure funding through research grants and private donations within Vietnam haven't been successful so far. Given the high cost of travel and accommodation, it is challenging for us to support Khanh's participation without external assistance. 

I firmly believe that attending Interspeech 2024 will be a pivotal moment in Khanh's career. It will boost his confidence and encourage him to continue his research. I sincerely hope that you will consider my request for sponsorship to enable Khanh to attend Interspeech 2024.

Thank you for considering my request. Your support would make a significant difference in Khanh's professional journey.

Sincerely,

Chau Thanh Duc
Head, Zalo AI Laboratory
ctduc@fit.hcmus.edu.vn


==> rebuttal.tex <==
Dear INTERSPEECH 2024 Technical Committees,

We are grateful for the insightful reviews and valuable feedback provided on Paper 1971. We appreciate the opportunity to address the reviewers' concerns.

Reviewer #4: Comparison with Similar Ideas (eg: Chunk-Based)
Our approach was indeed compared to the chunk-based method [13, 17, 18], a relevant technique. The results of this method are presented in Table 2 (A, C), and all experiments are clearly outlined in Section 3.1.

Reviewer #5: Experiment on additional dataset
While not mentioned, we also applied our techniques to a large-scale dataset (25.000 hours), achieving improvements in practical application. Unfortunately, due to confidentiality constraints, we were unable to include this dataset and its results in the end. However, we ensure the effectiveness of our proposal across various domains and datasets.

Reviewer #7: 
1. Confusion about AED Model Applicability
We acknowledge the confusion regarding the phrase "applicable for any streaming E2E ASR models built on attention-based architecture" for label-synchronous AED models. When referring to "streaming E2E ASR models," we meant inherently streamable models (time-synchronous) that don't require additional modules for streaming like CTC or RNN-T. AED models, with cross-attention, are not inherently streamable as the language part needs the whole speech for complete text output. While alignment modules like trigger attention can make AED streamable, combining it with TSCA is beyond this paper's scope. We will revise the phrase for clarity in the final version.
2. Latency Discussion
We regret the omission of absolute latency figures due to space constraints. Nonetheless, the influence of TSCA on relative latency can be inferred from the selection of chunk size and right context size.

We appreciate the reviewers for pointing out errors and providing suggestions for our paper, which will be duly addressed in the final version. 
Thank you for being so considerate!

